A Survey of Syntactic Modelling Structures in Biomedical Ontologies

Despite the large-scale uptake of semantic technologies in the biomedical domain, little is known about common modelling practices in published ontologies. OWL ontologies are often published only in the crude form of sets of axioms leaving the underlying design opaque. However, a principled and systematic ontology development life cycle is likely to be reflected in regularities of the ontology's emergent syntactic structure. To develop an understanding of this emergent structure, we propose to reverse-engineer ontologies taking a syntax-directed approach for identifying and analysing regularities for axioms and sets of axioms. We survey BioPortal in terms of syntactic modelling trends and common practices for OWL axioms and class frames. Our findings suggest that biomedical ontologies only share simple syntactic structures in which OWL constructors are not deeply nested or combined in a complex manner. While such simple structures often account for large proportions of axioms in a given ontology, many ontologies also contain non-trivial amounts of more complex syntactic structures that are not common across ontologies.

==> pic/hierarchyBranching.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,1282){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(946,1861){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(946,2439){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1087,484){\makebox(0,0){\strut{}$0$}}%
      \put(1974,484){\makebox(0,0){\strut{}$100$}}%
      \put(2862,484){\makebox(0,0){\strut{}$200$}}%
      \put(3750,484){\makebox(0,0){\strut{}$300$}}%
      \put(4637,484){\makebox(0,0){\strut{}$400$}}%
      \put(5525,484){\makebox(0,0){\strut{}$500$}}%
      \put(6412,484){\makebox(0,0){\strut{}$600$}}%
      \put(1540,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2330,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3750,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4011,154){\makebox(0,0){\strut{}Ontologies (grouped by category and ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5776,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6573,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{hierarchyBranching}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/hierarchyDepth.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,1282){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(946,1861){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(946,2439){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1087,484){\makebox(0,0){\strut{}$0$}}%
      \put(1974,484){\makebox(0,0){\strut{}$100$}}%
      \put(2862,484){\makebox(0,0){\strut{}$200$}}%
      \put(3750,484){\makebox(0,0){\strut{}$300$}}%
      \put(4637,484){\makebox(0,0){\strut{}$400$}}%
      \put(5525,484){\makebox(0,0){\strut{}$500$}}%
      \put(6412,484){\makebox(0,0){\strut{}$600$}}%
      \put(1540,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2330,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3750,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4011,154){\makebox(0,0){\strut{}Ontologies (grouped by category and ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5776,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6573,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{hierarchyDepth}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularityHierarchyDepthAxiom.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,943){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(682,1242){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,1542){\makebox(0,0)[r]{\strut{}$15$}}%
      \put(682,1841){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(682,2140){\makebox(0,0)[r]{\strut{}$25$}}%
      \put(682,2439){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(823,484){\makebox(0,0){\strut{}$0$}}%
      \put(1751,484){\makebox(0,0){\strut{}$100$}}%
      \put(2678,484){\makebox(0,0){\strut{}$200$}}%
      \put(3606,484){\makebox(0,0){\strut{}$300$}}%
      \put(4533,484){\makebox(0,0){\strut{}$400$}}%
      \put(5461,484){\makebox(0,0){\strut{}$500$}}%
      \put(6388,484){\makebox(0,0){\strut{}$600$}}%
      \put(1296,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2122,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3606,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(3879,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5323,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6120,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularityHierarchyDepthAxiom}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularityHierarchyDepthClassFrame.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,862){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(814,1037){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(814,1212){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(814,1387){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(814,1563){\makebox(0,0)[r]{\strut{}$50$}}%
      \put(814,1738){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(814,1913){\makebox(0,0)[r]{\strut{}$70$}}%
      \put(814,2088){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(814,2264){\makebox(0,0)[r]{\strut{}$90$}}%
      \put(814,2439){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(955,484){\makebox(0,0){\strut{}$0$}}%
      \put(1863,484){\makebox(0,0){\strut{}$100$}}%
      \put(2770,484){\makebox(0,0){\strut{}$200$}}%
      \put(3678,484){\makebox(0,0){\strut{}$300$}}%
      \put(4585,484){\makebox(0,0){\strut{}$400$}}%
      \put(5493,484){\makebox(0,0){\strut{}$500$}}%
      \put(6400,484){\makebox(0,0){\strut{}$600$}}%
      \put(1418,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2226,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3678,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(3945,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5350,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6147,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularityHierarchyDepthClassFrame}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularitySize.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1210,975){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(1210,1246){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1210,1518){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1210,1789){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1210,2060){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1210,2331){\makebox(0,0)[r]{\strut{}$1\times10^{6}$}}%
      \put(1350,484){\makebox(0,0){\strut{}$0$}}%
      \put(2198,484){\makebox(0,0){\strut{}$100$}}%
      \put(3046,484){\makebox(0,0){\strut{}$200$}}%
      \put(3893,484){\makebox(0,0){\strut{}$300$}}%
      \put(4741,484){\makebox(0,0){\strut{}$400$}}%
      \put(5589,484){\makebox(0,0){\strut{}$500$}}%
      \put(6436,484){\makebox(0,0){\strut{}$600$}}%
      \put(1783,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2537,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3893,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4143,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5033,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(5830,2665){\makebox(0,0)[r]{\strut{}(b)}}%
      \csname LTb\endcsname%%
      \put(6627,2665){\makebox(0,0)[r]{\strut{}(c)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{regularitySize}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularitySize2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(814,1572){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(814,2439){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(955,484){\makebox(0,0){\strut{}$0$}}%
      \put(1863,484){\makebox(0,0){\strut{}$100$}}%
      \put(2770,484){\makebox(0,0){\strut{}$200$}}%
      \put(3678,484){\makebox(0,0){\strut{}$300$}}%
      \put(4585,484){\makebox(0,0){\strut{}$400$}}%
      \put(5493,484){\makebox(0,0){\strut{}$500$}}%
      \put(6400,484){\makebox(0,0){\strut{}$600$}}%
      \put(1418,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2226,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3678,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(3945,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(4952,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(5749,2665){\makebox(0,0)[r]{\strut{}(b)}}%
      \csname LTb\endcsname%%
      \put(6546,2665){\makebox(0,0)[r]{\strut{}(c)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularitySize2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularitySizeClassFrame.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1210,975){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(1210,1246){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1210,1518){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1210,1789){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1210,2060){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1210,2331){\makebox(0,0)[r]{\strut{}$1\times10^{6}$}}%
      \put(1350,484){\makebox(0,0){\strut{}$0$}}%
      \put(2198,484){\makebox(0,0){\strut{}$100$}}%
      \put(3046,484){\makebox(0,0){\strut{}$200$}}%
      \put(3893,484){\makebox(0,0){\strut{}$300$}}%
      \put(4741,484){\makebox(0,0){\strut{}$400$}}%
      \put(5589,484){\makebox(0,0){\strut{}$500$}}%
      \put(6436,484){\makebox(0,0){\strut{}$600$}}%
      \put(1783,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2537,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3893,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4143,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5033,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(5830,2665){\makebox(0,0)[r]{\strut{}(b)}}%
      \csname LTb\endcsname%%
      \put(6627,2665){\makebox(0,0)[r]{\strut{}(c)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{regularitySizeClassFrame}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularitySizeClassFrames2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,1282){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(946,1861){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(946,2439){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1087,484){\makebox(0,0){\strut{}$0$}}%
      \put(1974,484){\makebox(0,0){\strut{}$100$}}%
      \put(2862,484){\makebox(0,0){\strut{}$200$}}%
      \put(3750,484){\makebox(0,0){\strut{}$300$}}%
      \put(4637,484){\makebox(0,0){\strut{}$400$}}%
      \put(5525,484){\makebox(0,0){\strut{}$500$}}%
      \put(6412,484){\makebox(0,0){\strut{}$600$}}%
      \put(1540,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2330,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3750,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4011,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(4979,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(5776,2665){\makebox(0,0)[r]{\strut{}(b)}}%
      \csname LTb\endcsname%%
      \put(6573,2665){\makebox(0,0)[r]{\strut{}(c)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularitySizeClassFrames2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularityStructureDepthAxiom.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,952){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,1200){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(682,1448){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(682,1695){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(682,1943){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,2191){\makebox(0,0)[r]{\strut{}$12$}}%
      \put(682,2439){\makebox(0,0)[r]{\strut{}$14$}}%
      \put(823,484){\makebox(0,0){\strut{}$0$}}%
      \put(1751,484){\makebox(0,0){\strut{}$100$}}%
      \put(2678,484){\makebox(0,0){\strut{}$200$}}%
      \put(3606,484){\makebox(0,0){\strut{}$300$}}%
      \put(4533,484){\makebox(0,0){\strut{}$400$}}%
      \put(5461,484){\makebox(0,0){\strut{}$500$}}%
      \put(6388,484){\makebox(0,0){\strut{}$600$}}%
      \put(1296,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2122,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3606,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(3879,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5323,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6120,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularityStructureDepthAxiom}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularityStructureSizeAxiom.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,1282){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(946,1861){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(946,2439){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1087,484){\makebox(0,0){\strut{}$0$}}%
      \put(1974,484){\makebox(0,0){\strut{}$100$}}%
      \put(2862,484){\makebox(0,0){\strut{}$200$}}%
      \put(3750,484){\makebox(0,0){\strut{}$300$}}%
      \put(4637,484){\makebox(0,0){\strut{}$400$}}%
      \put(5525,484){\makebox(0,0){\strut{}$500$}}%
      \put(6412,484){\makebox(0,0){\strut{}$600$}}%
      \put(1540,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2330,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3750,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4011,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5377,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6174,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularityStructureSizeAxiom}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/regularityStructureSizeClassFrame.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1078,1138){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(1078,1572){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1078,2005){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1078,2439){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1219,484){\makebox(0,0){\strut{}$0$}}%
      \put(2086,484){\makebox(0,0){\strut{}$100$}}%
      \put(2954,484){\makebox(0,0){\strut{}$200$}}%
      \put(3822,484){\makebox(0,0){\strut{}$300$}}%
      \put(4689,484){\makebox(0,0){\strut{}$400$}}%
      \put(5557,484){\makebox(0,0){\strut{}$500$}}%
      \put(6424,484){\makebox(0,0){\strut{}$600$}}%
      \put(1661,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2433,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3822,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4077,154){\makebox(0,0){\strut{}Ontologies (ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5404,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6201,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{regularityStructureSizeClassFrame}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/structureDepth.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7342.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1078,1138){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(1078,1572){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1078,2005){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1078,2439){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1219,484){\makebox(0,0){\strut{}$0$}}%
      \put(2086,484){\makebox(0,0){\strut{}$100$}}%
      \put(2954,484){\makebox(0,0){\strut{}$200$}}%
      \put(3822,484){\makebox(0,0){\strut{}$300$}}%
      \put(4689,484){\makebox(0,0){\strut{}$400$}}%
      \put(5557,484){\makebox(0,0){\strut{}$500$}}%
      \put(6424,484){\makebox(0,0){\strut{}$600$}}%
      \put(1661,2659){\makebox(0,0){\strut{}Atomic}}%
      \put(2433,2659){\makebox(0,0){\strut{}$\mathcal{EL}^{++}$}}%
      \put(3822,2659){\makebox(0,0){\strut{}Rich}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(473,1571){\rotatebox{90}{\makebox(0,0){\strut{}Number of Regularities}}}%
      \put(4077,154){\makebox(0,0){\strut{}Ontologies (grouped by category and ordered by size)}}%
      \csname LTb\endcsname%%
      \put(5794,2665){\makebox(0,0)[r]{\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(6591,2665){\makebox(0,0)[r]{\strut{}(b)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={367.10bp},height={144.00bp}]{structureDepth}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> relatedWork.tex <==
\section{Related Work}

Other frameworks for identifying regularities in ontologies in an automated man-
ner define regularities in terms of a combination of both syntactic properties as well
as qualitative properties such as frequency or similarity



\R{copy-pasted from old paper - rewrite this (use your thesis)}


One key difference to the approach used in this paper is the need of a parameter choice for what is considered 





A range of approaches for discovering syntax-based regularities in OWL ontologies have
been proposed.
First, agglomerative clustering has been used to identify commonalities between similar entities [8].
The notion of a replacement function can be interpreted as
a language abstraction. However, its use in the similarity distance measure effectively
reduces a set of axioms to a set of types of axioms. As a result, the proposed notion of
regularity based on clustering differs from regularities motivated in this work.

Second, frequent subtree mining over OWL axioms has been motivated by interpret-
ing them as (syntax) trees [5]. Furthermore, by using frequent itemset mining over identi-
fied regularities for axioms, regularities for sets of axioms are motivated. While frequent 
subtree mining aims to identify frequent structures, syntactic regularities based on lan-
guage abstractions do not. Language abstractions are primarily concerned with syntac-
tic properties and the corresponding notion for regularities is independent of any notion 
of frequency. The qualification of regularities in terms of being prevalent, i.e. capturing
frequently occurring syntactic structures, is a separate level of analysis.

\R{Not really sure about these}
Third, lexical naming conventions for OWL classes in combination with corresponding
structural relations in an ontology’s class hierarchy have been suggested to provide 
useful information w.r.t. an ontology’s underlying design [9].

Besides, approaches for discovering regularities from a given ontology alone, there 
also exists target-oriented approaches that aim to detect some predefined notion of pat-
terns [10, 11, 12]. Otherwise, there are surveys of ontologies discussing syntactic prop-
erties such as the prevalence of, for example, logical constructors [2, 13].

